Learning Cross-Context Entity Representations from Text

Language modeling tasks, in which words, or word-pieces, are predicted on the basis of a local context, have been very effective for learning word embeddings and context dependent representations of phrases. Motivated by the observation that efforts to code world knowledge into machine readable knowledge bases or human readable encyclopedias tend to be entity-centric, we investigate the use of a fill-in-the-blank task to learn context independent representations of entities from the text contexts in which those entities were mentioned. We show that large scale training of neural models allows us to learn high quality entity representations, and we demonstrate successful results on four domains: (1) existing entity-level typing benchmarks, including a 64% error reduction over previous work on TypeNet (Murty et al., 2018); (2) a novel few-shot category reconstruction task; (3) existing entity linking benchmarks, where we match the state-of-the-art on CoNLL-Aida without linking-specific features and obtain a score of 89.8% on TAC-KBP 2010 without using any alias table, external knowledge base or in domain training data and (4) answering trivia questions, which uniquely identify entities. Our global entity representations encode fine-grained type categories, such as Scottish footballers, and can answer trivia questions such as: Who was the last inmate of Spandau jail in Berlin?

==> one_page_examples.tex <==

\begin{figure*}[t]



    \begin{subtable}[b]{\textwidth}
    \small
    \centering
    \begin{tabular}{p{0.1\textwidth}|p{0.3\textwidth}|p{0.55\textwidth}}
        \toprule
        Category & Exemplars & Top 10 \\
        \midrule
        Action films & (1) Oblivion (2) Blood Diamond (3) Fight Club & \textbf{(1) The Bourne Supremacy} \textbf{(2) The Bourne Identity} (3) Zodiac \textbf{(4) Collateral} (5) Signs \textbf{(6) 2012} \textbf{(7) The Island} \textbf{(8) The Bourne Ultimatum} \textbf{(9) I Am Legend} \textbf{(10) Live Free or Die Hard} \\
        \hline
        American Biologists & (1) Michael Murphy Andregg (2) Mark Peifer (3) Mary Jane West-Eberhard & (1) Warder Clyde Allee \textbf{(2) Richard Lewontin} (3) Lancelot Hogben \textbf{(4) William Earnest Castle} \textbf{(5) Emile Zuckerkandl} (6) Lawrence Joseph Henderson (7) Alfred J. Lotka (8) Herbert Spencer Jennings (9) G. Evelyn Hutchinson \textbf{(10) H.J. Muller} \\
        \hline
        % Video games featuring female protagonists & (1) The Grinder (2) Final Fantasy XIII (3) Space Raiders & \textbf{(1) Final Fantasy X-2} \textbf{(2) Final Fantasy X} (3) Final Fantasy Type-0 \textbf{(4) Final Fantasty XIII-2} (5) Final Fantasy XV (6) Final Fantasy XII (7) Tales of Syphonia \textbf{(8) Dissidia Final Fantasy} (9) Kingdom Hearts coded (10) The World Ends with You \\
        % \hline
        Butterflies of Africa & (1) Neocoenyra bioculata (2) Phalanta madagascariensis (3) Mimacraea neokoton & (1) Neil Cazares-Thomas (2) Rhombophryne testudo (3) The Sick Child (4) Dillon Gordon (5) False smooth snake (6) Homoeosoma botydella (7) Northern Chinese softshel turtle (8) Catocala neogama (9) Hearths Like Ours (10) Iron Dragon \\
        \hline
        Giro d'Italia cyclists & (1) Paolo Savoldelli (2) Maxim Belkov (3) Pietro Bestetti & \textbf{(1) Giovanni Visconti}  \textbf{(2) Franco Pellizotti}  \textbf{(3) Gilberto Simoni} \textbf{(4) Michael Albasini} \textbf{(5) Paolo Bettini} \textbf{(6) Stefano Garzelli} \textbf{(7) Juan Antonio Flecha} \textbf{(8) Daniele Bennati}  (9) Thibaut Pinot \textbf{(10) Baden Cooke} \\
        \bottomrule
    \end{tabular}
    \caption{Top 10 predictions for a set of randomly selected Wikipedia, given 3 exemplars. Correct predictions are bolded.}
    \label{tab:category_preds}
    \end{subtable}
    
    \vspace{0.2cm}

\begin{subtable}[t]{\textwidth}
    \small
    \centering
    \begin{tabular}{p{0.55\textwidth}|p{0.4\textwidth}}
    \toprule
        Question & Top 5 Predictions  \\
    \midrule
        Who was the last inmate of Spandau jail in Berlin? & \textbf{(1) Rudolf Hess} (2) Adolf Hitler (3) Hermann Göring (4) Heinrich Himmler (5) Ernst Röhm \\
        \addlinespace
        Which fashionable London thoroughfare, about three quarters of a mile (1.2 km) long, runs from Hyde Park Corner to Marble Arch, along the length of the eastern side of Hyde Park? & \textbf{(1) Park Lane} (2) Piccadilly (3) Knightsbridge (4) Leicester Square (5) Tottenham Court Road \\
        \addlinespace
        In which Lake District town would you find the Cumberland Pencil Museum? & \textbf{(1) Keswick} (2) Hawkshead (3) Grasmere (4) Cockermouth (5) Ambleside \\
        \addlinespace
        The Wimbledon tennis tournament is held at which tennis club in London? & (1) Queen's Club \textbf{(2) All England Lawn Tennis and Croquet Club} (3) Wimbledon Championships (4) Stade Roland-Garros (5) Wentworth Club \\
        % \addlinespace
        % Which English city is known as `The Lace City'? & (1) Newcastle upon Tyne \textbf{(2) Nottingham} (3) Kingston upon Hull (4) Bradford (5) Leeds \\
        
        % What is the capital of the province of Manitoba, Canada? & \textbf{(1) Winnipeg} (2) Montreal (3) Saskatoon (4) Regina (5) Brandon \\
        % What is the name of the enzyme usually added to milk to coagulate it, to make "curds and whey"? & \textbf{(1) rennet} (2) pepsin (3) lipase (4) lactase (5) chymosin \\
        % \addlinespace
        % What is the name of the bay on the shore of which Rio de Janeiro sits? & \textbf{(1) Guanabara Bay} (2) Baía de Todos os Santos (3) Santa Catarina Island (4) Guaíba River (5) Lagoa Mirim \\
        % \hline
%         The left side of the heart pumps blood to all parts of the body, but the right side pumps blood to which organ in particular? & (1) liver (2) heart (3) kidney \textbf{(4) lung} (5) spleen \\
%         \addlinespace
%         In which country is the castle that gives the Habsburg dynasty its name? & (1) Austria \textbf{(2) Switzerland} (3) Andorra (4) Italy (5) Austrians \\
%         What is the name of the long running science program, produced by WGBH in Boston, on PBS, running from 1974 to the present? & \textbf{(1) Nova} (2) Radiolab (3) Mister Rogers' Neighborhood (4) This American Life (5) Horizon \\
% Columbia University, in the city of New York, was founded as King’s College by royal charter of which British monarch? & (1) George III of Great Britain \textbf{(2) George II of Great Britain} (3) William III (4) Anne of Great Britain (5) George I of Great Britain \\
% What term refers to a triangle with two equal sides? & \textbf{(1) isosceles triangle} (2) equilateral triangle (3) isosceles trapezoid (4) rhombus (5) kite \\
% What company is the world's largest auction house? & (1) Bonhams \textbf{(2) Christie's} (3) eBay (4) Sotheby's (5) Heritage Auctions \\
    \bottomrule
    \end{tabular}
    \caption{TriviaQA predictions from retrieval. Questions are randomly sampled, and top 5 ranking answers are shown. Correct answer in bold. Note that even when the model is wrong, the predictions are all of the correct type.}
    \label{tab:triviaqa_preds}
    \end{subtable}
    
    \caption{Qualitative results from evaluation.}

\end{figure*}

==> related.tex <==
% \section{Related work}
% \label{sec:related}

% \paragraph{Entity representations}

% Several works have tackled the problem of learning distributed representations of entities in a knowledge base (KB).
% Typical approaches rely on the (subject, relation, object) ontology of KBs like Freebase \citep{bollacker2008freebase}. These methods embed the entities and relations in vector space,  then maximize the score of observed triples against negative triples to do KB completion \citep{bordes2011learning, socher2013reasoning, yang2014embedding, toutanova2016compositional}.
% % Several works also consider extending representations beyond Euclidean embeddings, such as hyperbolic embeddings \citep{nickel2017poincare} or box embeddings \citep{vilnis2018box}. Such representations hold promise for integrating structured priors with embeddings, and while outside the scope of this work, should be explored in future work.

% There is relatively less work in learning entity representations directly from text.
% \citet{long2016leveraging} consider descriptions of entities, which limits the approach to entities in existing KBs.
% The contextual approach of word2vec \citep{mikolov2013distributed} has been extremely popular for word representations and has been applied to entities as well, but there has been little analysis of how effective such a method would be for answering the entity typing queries we study in this work.
% Most methods for entity representations that do use raw text will combine it with structure from an existing KB \citep{riedel2013relation, toutanova2015representing, hu2015entity} in an effort to leverage as much information as possible.
% While there may be gains to be had from using structure, our goal in this work is to isolate and understand the limits of inducing entity representations from raw text alone.

% \paragraph{Entity linking and mention typing}

% The motivating application of learning entity representations is typically entity linking or mention-level typing, as these tasks enable the use of KB resources for raw text.
% These tasks typically are set up with an entity mention in context, with the goal being to identify the entity (linking) or label it with types (typing).
% We note that our \ack task is reminiscent of entity linking,
% in particular to Wikification \citep{ratinov2011local, cheng2013relational}, where the task is to link mention text to Wikipedia pages.
% A key difference, however, is that we omit the entity mention;
% furthermore, our goal in defining the \ack~task is not to advance entity linking or typing per se, but to learn representations of entities that encapsulate the information in the mention contexts.

% Because of the similarity of standard tasks to \ack, several of our modeling choices are the same.
% Standard neural models embed the entity mention and context in an end-to-end network that can be used to predict types \citep{yaghoobzadeh2015corpus, shimaoka2016attentive}, link the entity mention \citep{sun2015modeling, yamada2016joint, gupta2017entity, murty2018hierarchical}, or even generate descriptions of the entity \citep{ishiwatari2018learning}.

% Additionally, we note that we consider entity typing of \ack~from a \emph{global} perspective instead of the more common context-dependent entity mention typing tasks \citep{ling2012fine, choi2018ultra}. 
% We are interested in identifying context-independent types of entities for applications in automated knowledge base construction.


% % \subsection{External knowledge}


% % Several works have identified the problem of using external knowledge to augment neural networks for inference.
% % Most of these works use 
% % \citet{weissenborn2017dynamic} retrieve Wikipedia entities and update the word embeddings of their model to improve results in question answering.
% % \citet{das2018multi} consider open domain question answering where knowledge is represented as paragraph encodings, and relevant paragraphs are retrieved and passed to a machine reading model.

% % Neural models for question answering have been extensively studied, from using pure retrieval \citep{iyyer2014neural} to span classification \citep{seo2017bidirectional, clark2018simple} (MORE CITATIONS NEEDED)



% \paragraph{Fill-in-the-blank tasks}


% Our \ack~task is similar to word2vec \citep{mikolov2013distributed}, and can be compared to the task of language modeling \citep{jozefowicz2016exploring}.
% Several works have used language modeling-style losses for pretraining networks from semi-supervised or unsupervised data sources \citep{dai2015semi, howard2018universal, peters2018deep, radford2018improving, joshi2018pair2vec, devlin2018bert}.
% Our work borrows the idea of large-scale learning, but we focus on entities, whose names can often span multiple tokens.

% Other works have considered tasks like ours. \citet{bisk2016evaluating} introduce the SPADES fill-in-the-blank task, but their dataset is heavily reliant on Freebase and is unsuited for general evaluation.
% \citet{long2017world} consider a similar fill-in-the-blank task as ours, which they frame as rare entity prediction.
% However, their model does not aim to learn entity representations.
% \citet{yamada2016joint} also use Wikipedia hyperlinks to do fill-in-the-blank training of entities, but they focus on the entity linking task instead of the entity representations.

==> related_emnlp.tex <==
\section{Related work}
\label{sec:related}

\paragraph{Entity linking}
The most widely studied entity-level task is entity linking---mapping each entity mention onto a unique entity identifier. 
The Wikification task \citep{ratinov2011local, cheng2013relational}, in particular, is similar to the work presented in this paper, as it requires systems to map mentions to the Wikipedia pages describing the entities mentioned. 
There is significant previous work that makes use of neural context and entity encoders in downstream entity linking systems \citep{sun2015modeling, yamada2016joint, yamada-etal-2017-learning, gupta2017entity, murty2018hierarchical,kolistas2018end}, but that previous work focuses solely on discriminating between entities that match a given mention according to an external alias table. Here we go further in investigating the degree to which \ack~can capture world knowledge about entities.

\paragraph{Mention-level entity typing}
Another well studied task is mention-level entity typing \citep[e.g.][]{ling2012fine, choi2018ultra}. 
In this task, entities are labeled with types that are supported by the immediate textual context. 
For example, given the sentence {\it `Michelle Obama attended her book signing'}, Michelle Obama should be assigned the type {\it author} but not {\it lawyer}. 
Subsequently, mention-level entity typing systems make use of contextualized representations of the entity mention, rather than the global entity representations that we focus on here.
% Here, we focus instead on corpus wide \emph{entity-level typing}.

\paragraph{Entity-level typing}
An alternative notion of entity typing is entity-level typing, where each entity should be associated with all of the types supported by a corpus.
\citet{yaghoobzadeh2015corpus} and \citet{murty2018hierarchical} introduce entity-level typing tasks, which we describe more in Section~\ref{sec:entity_typing_results}. 
Entity-level typing is an important task in information extraction, since most common ontologies make use of entity type systems. Such tasks provide a strong method of evaluating learned global representations of entities.

\paragraph{Using knowledge bases} 
There has been a strong line of work in learning representations of entities by building knowledge base embeddings \citep{bordes2011learning, socher2013reasoning, yang2014embedding, toutanova2016compositional, vilnis2018box}, and by jointly embedding knowledge bases and information from textual mentions \citep{riedel2013relation, toutanova2015representing, hu2015entity}.
\citet{das2017question} extended this work to the {\sc spades} fill-in-the-blank task \citep{bisk2016evaluating}, which is a close counterpart to \ack's training setup.
However, we note that all examples in {\sc spades} correspond to a fully connected sub-graph in Freebase~\cite{bollacker2008freebase}. 
Subsequently, the contents 
%of {\sc spades}
are very limited in domain and \citet{das2017question} show that it is essential to use the contents of Freebase to do well on this task. 
We consider the unconstrained TriviaQA task \citep{joshi2017triviaqa}, introduced in Section~\ref{sec:trivia-qa}, to be a better evaluation for open domain knowledge representations.

\paragraph{Fill-in-the-blank tasks} 
There has been significant previous work in using fill-in-the-blank losses to learn context independent word representations \citep{mikolov2013distributed}, and context-dependent word and phrase representations \citep{dai2015semi,peters2018deep,radford2018improving,devlin2018bert}.
Cloze-style tasks, in which a system must choose which of a few entities best fill a blanked out span, have also been proposed as a method of evaluating reading comprehension \citep{Hermann:15, long2016leveraging, Onishi:16}. 
For entities, \citet{long2017world} consider a similar fill-in-the-blank task as ours, which they frame as rare entity prediction.
\citet{yamada2016joint} and \citet{yamada-etal-2017-learning} train entity representations using a fill-in-the-blank style loss and a bag-of-words representation of mention contexts. 
\citet{yamada2016joint, yamada-etal-2017-learning}~in particular take an approach that is very similar in motivation to \ack, but which focuses on learning entity representations for use as features in downstream classifiers that model non-linear interactions between a small number of candidate entities. 
In Section~\ref{sec:category_completion}, we show that \cite{yamada-etal-2017-learning}'s entity embeddings are good at capturing broad entity types such as {\it Tennis Player} but less good at capturing more complex compound types such as {\it Scottish Footballers}. 
In Section~\ref{sec:entity_linking_results}, we also show that by performing nearest neighbor search over the 818k entities in the TAC knowledge base, \ack can surpass \citealt{yamada-etal-2017-learning}'s performance on the \tac~entity linking benchmark \citep{Ji10overviewof}. This is despite the fact that \citeauthor{yamada-etal-2017-learning} massively restrict the linking search space with an externally defined alias table, and incorporate task-specific hand-engineered features. On the CoNLL-Aida benchmark, we show that \ack surpasses \citealt{yamada-etal-2017-learning} and matches \citealt{Raiman2018-hm} without using any entity linking-specific features.

% \begin{comment}

% \paragraph{Entity representations}

% Several works have tackled the problem of learning distributed representations of entities in a knowledge base (KB).
% Typical approaches rely on the (subject, relation, object) ontology of KBs like Freebase \citep{bollacker2008freebase}. These methods embed the entities and relations in vector space,  then maximize the score of observed triples against negative triples to do KB completion \citep{bordes2011learning, socher2013reasoning, yang2014embedding, toutanova2016compositional}.
% % Several works also consider extending representations beyond Euclidean embeddings, such as hyperbolic embeddings \citep{nickel2017poincare} or box embeddings \citep{vilnis2018box}. Such representations hold promise for integrating structured priors with embeddings, and while outside the scope of this work, should be explored in future work.

% There is relatively less work in learning entity representations directly from text.
% \citet{long2016leveraging} consider descriptions of entities, which limits the approach to entities in existing KBs.
% The contextual approach of word2vec \citep{mikolov2013distributed} has been extremely popular for word representations and has been applied to entities as well, but there has been little analysis of how effective such a method would be for answering the entity typing queries we study in this work.
% Most methods for entity representations that do use raw text will combine it with structure from an existing KB \citep{riedel2013relation, toutanova2015representing, hu2015entity} in an effort to leverage as much information as possible.
% While there may be gains to be had from using structure, our goal in this work is to isolate and understand the limits of inducing entity representations from raw text alone.

% \paragraph{Entity linking and mention typing}

% The motivating application of learning entity representations is typically entity linking or mention-level typing, as these tasks enable the use of KB resources for raw text.
% These tasks typically are set up with an entity mention in context, with the goal being to identify the entity (linking) or label it with types (typing).
% We note that our \ack task is reminiscent of entity linking, in particular to Wikification \citep{ratinov2011local, cheng2013relational}, where the task is to link mention text to Wikipedia pages.
% A key difference, however, is that we omit the entity mention; furthermore, our goal in defining the \ack~task is not to advance entity linking or typing per se, but to learn representations of entities that encapsulate the information in the mention contexts.

% Because of the similarity of standard tasks to \ack, several of our modeling choices are the same.
% Standard neural models embed the entity mention and context in an end-to-end network that can be used to predict types \citep{yaghoobzadeh2015corpus, shimaoka2016attentive}, link the entity mention 
% \citep{sun2015modeling, yamada2016joint, gupta2017entity, murty2018hierarchical}
% , or even generate descriptions of the entity \citep{ishiwatari2018learning}.

% Additionally, we note that we consider entity typing of \ack~from a \emph{global} perspective instead of the more common context-dependent entity mention typing tasks \citep{ling2012fine, choi2018ultra}. 
% We are interested in identifying context-independent types of entities for applications in automated knowledge base construction.


% % \subsection{External knowledge}


% % Several works have identified the problem of using external knowledge to augment neural networks for inference.
% % Most of these works use 
% % \citet{weissenborn2017dynamic} retrieve Wikipedia entities and update the word embeddings of their model to improve results in question answering.
% % \citet{das2018multi} consider open domain question answering where knowledge is represented as paragraph encodings, and relevant paragraphs are retrieved and passed to a machine reading model.

% % Neural models for question answering have been extensively studied, from using pure retrieval \citep{iyyer2014neural} to span classification \citep{seo2017bidirectional, clark2018simple} (MORE CITATIONS NEEDED)



% \paragraph{Fill-in-the-blank tasks}


% Our \ack~task is similar to word2vec \citep{mikolov2013distributed}, and can be compared to the task of language modeling \citep{jozefowicz2016exploring}.
% Several works have used language modeling-style losses for pretraining networks from semi-supervised or unsupervised data sources \citep{dai2015semi, howard2018universal, peters2018deep, radford2018improving, joshi2018pair2vec, devlin2018bert}.
% Our work borrows the idea of large-scale learning, but we focus on entities, whose names can often span multiple tokens.

% Other works have considered tasks like ours. \citet{bisk2016evaluating} introduce the SPADES fill-in-the-blank task, but their dataset is heavily reliant on Freebase and is unsuited for general evaluation.
% \citet{long2017world} consider a similar fill-in-the-blank task as ours, which they frame as rare entity prediction.
% However, their model does not aim to learn entity representations.
% \citet{yamada2016joint} also use Wikipedia hyperlinks to do fill-in-the-blank training of entities, but they focus on the entity linking task instead of the entity representations.

% \end{comment}
